Iteratively Refined Behavior Regularization for Offline Reinforcement Learning

One of the fundamental challenges for offline reinforcement learning (RL) is ensuring robustness to data distribution. Whether the data originates from a near-optimal policy or not, we anticipate that an algorithm should demonstrate its ability to learn an effective control policy that seamlessly aligns with the inherent distribution of offline data. Unfortunately, behavior regularization, a simple yet effective offline RL algorithm, tends to struggle in this regard. In this paper, we propose a new algorithm that substantially enhances behavior-regularization based on conservative policy iteration. Our key observation is that by iteratively refining the reference policy used for behavior regularization, conservative policy update guarantees gradually improvement, while also implicitly avoiding querying out-of-sample actions to prevent catastrophic learning failures. We prove that in the tabular setting this algorithm is capable of learning the optimal policy covered by the offline dataset, commonly referred to as the in-sample optimal policy. We then explore several implementation details of the algorithm when function approximations are applied. The resulting algorithm is easy to implement, requiring only a few lines of code modification to existing methods. Experimental results on the D4RL benchmark indicate that our method outperforms previous state-of-the-art baselines in most tasks, clearly demonstrate its superiority over behavior regularization.

==> tex/related.tex <==

\section{Related Work}
% policy constraint
In the offline RL, policy constraint is the most straightforward and intuitive method for avoiding the issue of distributional shift. The core idea is to ensure that the learning policy cannot be too far away from the behavioral policy. Based on BC~\cite{bain1995framework} that actions are selected from the dataset and cloned, some attempts are made to ensure that the distribution is bounded by carefully parameterizing the learning policy~\cite{fujimoto2019off,ghasemipour2021emaq}. In addition, several works explicitly apply divergence penalty terms to help adjust the learning policy, e.g., KL divergence~\cite{nair2020awac} and MMD distance~\cite{kumar2019stabilizing}. A general framework is proposed to evaluate these divergence-dependent methods~\cite{wu2019behavior}. More recently, other problem-specific regularization terms have been found to be more effective. These can be accomplished by adding a simple behavior cloning term that produces exceptional performance~\cite{fujimoto2021minimalist}, regularizing behavior density directly to put more precise constraints~\cite{wu2022supported}, or generalizing OOD samples within a convex hull of training data using the distance function~\cite{li2022distancesensitive}.

The policy constraint of these works can generally be assumed to be implemented based on the behavioral cloned policy. When data quality is high, BC is capable of achieving competitive performance thus the above methods can achieve satisfactory performance. However, a naive behavioral cloning approach is unworkable when the dataset is collected by a sub-optimal or multi-modal policy.
To improve the quality of the behavioral policy used for constraint, several alternatives have been proposed. Weighted BC is a way to clone only the available best behavioral actions by down-weighting low-quality data or simply discarding them. Many works evaluate the relative advantages of transitions and rely on them to filter the most promising ones in the dataset~\cite{wang2020critic,brandfonbrener2021quantile,brandfonbrener2021offline,kostrikov2022offline} or pick the trajectory samples based on Monte Carlo returns~\cite{peng2019advantage,chen2020bail,siegel2020keep}.
Conditional BC introduces an additional condition as the input of BC. \cite{emmons2022rvs} demonstrates the effectiveness of conditional BC and shows that an appropriate conditional variable is crucial when offline RL takes a supervised learning approach. These approaches use return-to-go as a condition to make better sequential decisions~\cite{chen2021decision,janner2021offline} or select a future goal state as a condition and can extract the behavior of reaching the goal from sparse rewards~\cite{emmons2022rvs,yang2022rethinking}. Furthermore, a recent research~\cite{xu2022a} learns guide-policy and execute-policy separately and uses the state generated by guide-policy to steer where execute-policy goes.  ~\cite{wang2022diffusion} proposed to employ the diffusion model as a highly expressive policy class and use it to constrain the learning policy, which achieves the state-of-the-art performance among the policy constraint offline RL methods. PSPO shares the same idea of improving the policy used for constraints, but PSPO does not need to employ complex policy models such as diffusion model, still achieving similar or even better performance while greatly saving computational overhead. 


